Sequential Modeling with Multiple Attributes for Watchlist Recommendation in E-Commerce

In e-commerce, the watchlist enables users to track items over time and has emerged as a primary feature, playing an important role in users' shopping journey. Watchlist items typically have multiple attributes whose values may change over time (e.g., price, quantity). Since many users accumulate dozens of items on their watchlist, and since shopping intents change over time, recommending the top watchlist items in a given context can be valuable. In this work, we study the watchlist functionality in e-commerce and introduce a novel watchlist recommendation task. Our goal is to prioritize which watchlist items the user should pay attention to next by predicting the next items the user will click. We cast this task as a specialized sequential recommendation task and discuss its characteristics. Our proposed recommendation model, Trans2D, is built on top of the Transformer architecture, where we further suggest a novel extended attention mechanism (Attention2D) that allows to learn complex item-item, attribute-attribute and item-attribute patterns from sequential-data with multiple item attributes. Using a large-scale watchlist dataset from eBay, we evaluate our proposed model, where we demonstrate its superiority compared to multiple state-of-the-art baselines, many of which are adapted for this task.

==> framework-old.tex <==
\section{Recommendation Framework}
\label{sec:framework}
We now describe our \wl recommendation (WLR) framework. We start with problem formulation (Section~\ref{sec:formulation}), where we further cast the WLR task as a specialized SR task (Section~\ref{sec:SR}). We then propose a Transformer-based recommendation model, which employs a novel Attention2D mechanism capable of encoding item attribute-rich input sequences (Section~\ref{sec:model}). 


\subsection{Problem Formulation}
\label{sec:formulation}
The \wl recommendation task can be modeled as a special case of the sequential recommendation (SR) task~\cite{wang2019sequential}, with a distinction that, at every possible moment, there is only a limited, yet dynamic, valid set of watched items that need to be considered.  Using the user's historical interactions with \wl items and her recently viewed items (RVIs), our goal is, therefore, to predict which items in the current user's \wl will be clicked. A user's click on a \wl item would imply that the user has regain her interest in that item. Moreover, we wish to leverage the fact that watched items are dynamic, having attributes whose values may change over time (e.g., price), and therefore, may imply on a change in user's preferences. 

Formally, let $\U$ be the set of all users, and let $\I$ be the set of all recommendable items. At any given point of time, the current \wl of any user in $\U$ may include any item from $\I$.
For a given user $u\in{\U}$, let $\WL^u_t\subseteq{\I}$ denote the set of items in the user's \wl at the time of $t$-th interaction with her \wl, termed also hereinafter a ``\emph{\wl snapshot}''. We further denote $m_t=|\WL^u_t|$ the number of items in a given snapshot. A user may click on any item in $\WL^u_t$, which leads the user to the item's page; also termed a ``view item'' (VI) event. %We assume that once the user views a recommended watched item, a new \wl session starts immediately after she gets back to her \wl.  
VI events may also occur independently of items in the user's \wl; e.g., the user views an  item in $\I$ following some search result or directed to the item's page through some other organic recommendation module, etc. Let $\VI^u_t\subseteq{\I}$ further denote a possible sequence of items viewed by user $u$ between the $t$-th and $t+1$-th interactions with her \wl.  
The user's history prior to her next \wl interaction to be considered for item recommendation is given by the sequence of \wl snapshots and recently viewed item (RVI) events: $\H^u(t)=\left(\WL^u_1,\VI^u_1,\ldots,\WL^u_t,\VI^u_t\right)$, where $t \in [1,\ldots,T_u]$ and $T_u$ denotes the number of historical \wl snapshots recorded for user $u$. While viewed items in each $\VI^u_t$ are ordered by time, there is no obvious prior order for items in each snapshot $\WL^u_t$. Therefore, to enforce an order also on items in \wl snapshots, we assume that such items are ordered by the time they were added by the user to her \wl (i.e., newly added items are ordered first). As we shall demonstrate in our experiments, such prior ordering actually serves by itself as a strong baseline. % to beat. 

%\hr{note that you don't use the attribute definition elsewhere...hence we don't need to formally define this set..I believe it is obvious from context. The less notations, the better.} Each item $v\in{\V}$ occurrence in a given \wl session or RVI event is associated with as set of $C$ categorical attributes (for the full list of attributes refer to Appendix \ref{<TODO>}). An item attribute's value may change over time (e.g., price, quantity, item shipment terms, seller ID, etc.). 

 Additionally, each item $v^u_{t,i}\in\WL^u_t$ ($1\leq{i}\leq{m_t}$; $1\leq{t}\leq{T_u}$) is associated with a label $y^u_{t,i}$ that denotes whether user $u$ clicked on $v^u_{t,i}$ (i.e., $y^u_{t,i}=1$) or not (i.e., $y^u_{t,i}=0$). Since item clicks in our setting are very sparse, it is problematic to represent items solely by their item-ID as has been done so far in most related literature~\cite{wang2019sequential}. Alternatively, in this work, we represent an item based on its attributes. Such a representation allows our model to generalize based on item’s explicit attributes rather than having to train an unique/independent representation for each item, thus addressing the sparsity and item cold-start problems\footnote{We note that, due to the nature of the WLR task, user cold-start is not an issue, since users are explicitly modeled by their \wl.}. It is further worth noting that, while in most previous works items remain static, as item-IDs are basically fixed, in our case, items are dynamic, having attributes that may change over time. 
 
Using the above definitions, for a given user $u\in{U}$, and interaction index $t \in [1,\ldots,T_u]$, the WLR task input is $H^u(t)$, $\WL^u_{t+1}$ and labels $y^u_{l,i}$ ($\forall v^u_{l,i}\in{\WL^u_{l}}$; $1\leq{i}\leq{m_{l}}$; $1\leq{l}\leq{t}$). The task's goal is, therefore, to predict: $y^u_{t+1,i}$;  $\forall v^u_{t+1,i}\in{\WL^u_{t+1}}$ ($1\leq{i}\leq{m_{t+1}}$), i.e., which items in the next \wl snapshot $\WL^u_{t+1}$ may be clicked by $u$. Therefore, at service time, we wish to recommend to the user the top-$k$ items in $\WL^u_{T_u+1}$ with the highest click likelihood.

\subsection{Sequence Representation}\label{sec:SR}
As the first step towards addressing the WLR task, we now cast it as a SR task. %Yet, to remind, compared to most previous works on sequence-based reocommendation~\cite{TODO}, whose primary goal is to predict the identity of the next item the user will interact with, our goal is to predict which items in a given (closed) set of user's watched items will be click by the user and rank them accordingly.  
To simplify notations, from now on, we assume all information regards a specific user $u\in \U$; hence, unless explicitly needed for clarity, we omit the user index $u$. % and neglect indexing for a user.
%To this end, 

Given a user, we flatten her history $\H(t)$ together with the next \wl snapshot $\WL_{t+1}$ and obtain the following item sequence (starting from the first history \wl snapshot $\WL_{1}$):  
\[
\S(t)=
%\underbrace{v_{1,1},\ldots,v_{1,m_1}}_{\WL_1}, %\underbrace{v'_{1,1}, \ldots, v'_{1,n_1}}_{\VI^1} \cdots
\cdots\underbrace{v_{t,1},\ldots,v_{t,m_t}}_{\WL_t}, \underbrace{v'_{t,1},\ldots,v'_{t,n_t}}_{\VI_t},
% \]
% \[
\underbrace{v_{t+1,1},\ldots,v_{t+1,m_{t+1}}}_{\WL_{t+1}\ (prediction)}
\]
Here, to distinguish between watched and viewed items, we use the notations $v$ and $v'$, respectively. $m_{l}$ and $n_{l}$ (for $1\leq{l}\leq{t+1}$) denote the number of items in $\WL_{l}$ (the $l$-th \wl snapshot) and $\VI_{l}$ (the $l$-th sequence of viewed items), respectively. Each item $v,v'\in S(t)$ is associated with a rich set of $C$ categorical attributes (e.g., item price, category, seller-ID, sale type, condition, etc.), whose values may change over time. For each item $v,v'\in S(t)$, we further add several snapshot-based attributes such as the relative snapshot position ($l$) and month and day of user interaction, item's relative position within a snapshot or VI sequence, etc (the full list of attributes is described in Section~\ref{sec:dataset}).

The straightforward sequence representation is to consider only items that the user clicked or viewed (either after explicitly clicking on a watched item or implicitly visiting the viewed item page through a different source). Recall that, our task is to rank the current user's \wl items based on their likelihood to be clicked by the user.  Since we wish to  model the interplay between various \wl items and their effect on user's preferences per snapshot, we choose to leverage the representation of all items (clicked and not clicked) that are tracked by the user over time. %\hr{Uriel, that's a new part I added to mention the repetition modeling} 
Furthermore, we note that, a user may click (or may not) on the same \wl item in different \wl snapshots. Modeling such repetitive behavior has been shown to be highly effective in other SR tasks~\cite{10.1145/3121050.3121061,sar2018collaborative}. %\hr{this is repetition of what we say already above} Similar to item's representation in $S(t)$, the current watched items are also represented by the set of $C$ attributes. Note again, at inference time, the attribute values of any watched item may have changed since the last \wl snapshot. 

\subsection{Recommendation Model}\label{sec:model}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{model-detailed.pdf}
\caption{Watchlist recommendation model using Transformer with Attention2D layer. Note that the input sequence starts from the first \wl snapshot $\WL_{1}$, yet is omitted for simplification.}
\label{fig:model}
\end{figure}

Our WLR model extends the Transformer~\cite{vaswani2017attention} architecture for handling sequences with items that include several categorical attributes as in the case of \wl items. Using such an architecture allows us to capture high-order dependencies among items and their attributes with minimum loss of semantics and a reasonable model complexity. The model's network architecture is depicted in Figure~\ref{fig:model}. The network includes three main layers, namely, \emph{Embedding} layer, \emph{Attention2D} layer and \emph{Prediction} layer. We next describe the details of these three layers.

\subsection{Embedding Layer}
\label{sec:embedding}
 A common modeling choice in most related literature~\cite{wang2019sequential}, is to represented user's sequence as the sequence of item-ids %with whom the user has interacted 
(including those in the next \wl snapshot for prediction): 
$\S(t) = \left(ID_1=ID(v_{1,1}),\ldots,ID_N=ID(v_{t+1,m_{t+1}})\right)$,
further having $N=m_{t+1}+\sum_{l=1}^{t}(m_{l}+n_{l})$ as the total items in $\S(t)$. These item-ids are typically embedded into a corresponding sequence of $d$-dimensional vectors $\E = (\e_1,\ldots,\e_N); \forall{i}:\e_i \in \RR^{d} $ using an embedding dictionary and serve as input representation to neural-network models. 
However, such a representation has two main disadvantages. Firstly, it is prone to cold-start problems as items that never appear during training must be discarded or embedded as an `unknown' item. Secondly, items that only appear once or a few times during training are at high risk of over-fitting by the training process memorizing their spurious labels.
Such sparsity issues are particularly present in our data (as will be discussed in Section~\ref{sec:dataset}), prompting us to represent an item as a collection of attributes, rather than only an item-id. Such an approach is less prone to sparsity and over-fitting, as the model learns to generalize based on item-attributes.

Following our choice for item representation, we now assume that each item in the user's sequence $v,v'\in\S(t)$ is represented by $C$ attributes: $[a_1,\ldots,a_C]$. Therefore, the input to our model is a 2D-array of item attributes $S(t) = [a]_{i,j}$; where  $i \in [1,\ldots,N], j \in [1,\ldots,C]$. %Here $M$ is the number items in the user's history and $C$ is the number of possible attributes. 
Hereinafter, we shall refer to the first axis of $S(t)$ as the \textit{sequence} (item) dimension and to its second axis as the \textit{channel} (attribute) dimension. We further assume all attributes are categorical, and those that are not, are binned using 100 equal-sized bins over the histogram equalization\footnote{\url{https://en.wikipedia.org/wiki/Histogram_equalization}}. Again, the full list of attributes is described in Section~\ref{sec:dataset}. %For a description of the full attributes list we use, please refer to Table \ref{table:attributes}) \hr{this should change to section number}.

The first layer of our model is an embedding layer with keys for all possible attribute values in our data. Therefore, by applying this layer on the user's sequence $\S(t)$, we obtain a 2D-array of embedding vectors $\E = [e]_{i, j} = Embd([a]_{i, j})$. Note that, since each item attribute embedding by itself is a $d$-dimensional vector, $\E\in\RR^{N\times{C}\times{d}}$ is actually a 3D-array. $\E$ is next fed into a specially \emph{modified Transformer} layer which is the main processing layer of our model and whose details are presented next. 

\subsection{Modified Transformer}
\label{sec:modified_transformer}
In the past, a number of architecture alternatives have been successfully employed to handle sequential data, such as GRU~\cite{hidasi2016sessionbased}, CNN~\cite{10.1145/3159652.3159656} and attention-based Transformers~\cite{kang2018self,sun2019bert4rec}, where all take in a sequence of vectors as input. 
However, in our case, we do not have a 1D-sequence of vectors but rather a 2D-array representing a sequence of ordered attribute collections. As Transformers were shown to demonstrate state-of-the-art performance in handling sequential data in general~\cite{vaswani2017attention} and sequential recommendation data specifically \cite{kang2018self, sun2019bert4rec, zhou2020s3}, we choose to employ Transformers and extend the \emph{Attention Mechanism} of the Transformer to handle 2D-input sequences, rather than a 1D-input sequence.

Since the vanilla attention model employed by existing Transformer architectures cannot be directly used for 2D-data, different pooling techniques were devised to reduce the channel dimension and produce a 1D-sequence as an input for the Transformer. For example, in BERT \cite{kenton2019bert},  token, position and sentence embeddings are summed before being fed into the Transformer Encoder. Other alternatives to summation were explored such as averaging, concatenation, or a secondary Transformer layer (e.g.,~\cite{10.1145/3326937.3341261,zhang2019feature}). Yet, most of these approaches suffer from a reduction in data representation happening prior to applying the attention workhorse. This makes it harder for the attention mechanism to learn rich attention patterns. 
An exception is the concatenation approach that sidesteps this problem but produces very long vectors, which in turn, requires Transformer layers to have a large input dimension making them needlessly large.

As an alternative, we next propose \textbf{\Atd} -- a dedicated novel attention block that is natively able to handle 2D-inputs in an efficient way. Such an extended attention mechanism will allow us to learn better attention patterns without significantly increasing the architecture size.

\subsection{Attention2D}
\label{sec:attention2d}

% \begin{figure*}
% \begin{subfigure}{.33\textwidth}
%   \centering
%   \includegraphics[width=0.6\textwidth]{Attention2D.pdf}
% \end{subfigure}%
% \begin{subfigure}{.4\textwidth}
%   \centering
%   \includegraphics[width=0.6\textwidth]{MultiHead2D.pdf}
% \end{subfigure}
% \begin{subfigure}{.26\textwidth}
%   \centering
%   \includegraphics[width=0.6\textwidth]{ScaledTensorDotProduct.pdf}
% \end{subfigure}
% \caption{\hr{this figure still has "Tensor"...need to modify} (left) The full \Atd architecture. (middle) The Multi-Head \Atd block. (right) The Scaled Tensor-Dot-Product block. The inspiration for the \Atd block is from the original attention block presented at \cite{vaswani2017attention}, where changes were made in order to be able to handle 3D tensors as input.}
% \label{fig:architecture}
% \end{figure*}
    
We now describe in detail our modified attention block, referred to as \Atd. For comparison to the vanilla Transformer model, we encourage the reader to refer to~\cite{vaswani2017attention}.
An attention block maps a query ($\Q$) and a set of key ($\K$) - value ($\V$) pairs to an output, where the query, keys, values, and output are all vectors \cite{vaswani2017attention}. 
The \Atd block in turn receives a 2D-array of vectors, representing a sequence of ordered item attribute collections and computes the attention between all item-attributes while enabling different semantics per channel to better capture both channel interactions and differences.
This way, one attribute of a specific item can influence another attribute of a different item regardless of other attributes, making it possible to learn high-order dependencies between different items and attributes. For instance, in our use-case, the price preferences of a user, captured by the price channel can be computed using attention both to previously clicked item prices and to past viewed items of sellers correlated with pricey or cheap items. 

The full \Atd block is illustrated in  Figure~\ref{fig:model}. We now provide a detailed description of its implementation. In all that follows, we refer to our inputs as 2D-arrays of vectors for ease of explanation. In practice, our model was implemented using high-order tensors, and tensor operations which are efficient, batched extensions of the vector and matrix operations described here.


\subsubsection{\Ltd}
\label{sec:fc2d}
The input to our model is a 2D-array of input vectors, generally denoted hereinafter $\X = [\x]_{i,j}$ (and specifically in our model's input $\X=\E$). Our model requires operations acting on such 2D-arrays throughout. To this end, we first define two extensions of standard linear neural network layers:

\begin{equation}
\begin{split}
\Ltd_{W}(\X) = \W_j [\x]_{i,j} \\
\Ltdb_{W,b}(\X) = \W_j [\x]_{i,j} + b_j,
\end{split}
\end{equation}

where $\W = [W_1,\ldots,W_C]; b = [b_1,\ldots,b_C]$ and $\W_j \in \RR^{d \times d}; b_j \in \RR^{d}$ are trainable parameters per channel $1\leq j\leq C$. These operations define a linear layer (with or without bias) with different trainable parameters per channel and shall allow the model to facilitate interactions between different channels while preserving the unique semantics of each channel.  %Note that, the two dimension sizes $d$ and $d'$ can be different. Yet, in our implementation we used the same dimension size \ye{maybe: Yet, in our implementation we used a fixed dimension size throughout our model. But make sure this is correct. If i'm not mistaken d'=d/k prior to the multi-head attention layer with k heads?} \hr{Uriel, please confirm, if that's true, please add a mention of this fact in the multi-head subsection. Cool catch Yotam!}.  

We start by mapping our input ($\E$) into three 2D-arrays of query $\Q = [\q]_{i,j}$, key $\K = [\k]_{i,j}$ and value $\V = [\v]_{i,j}$ vectors corresponding to each input. We do so by applying three \Ltd layers:

$$\Q = \Ltd_{Q}(\X) \ ; \ \K = \Ltd_{K}(\X) \ ; \ \V = \Ltd_{V}(\X)$$


\subsubsection{\AtdH}
\label{sec:tensordot}
We next describe the core part of our proposed attention mechanism, which is used to compute a transformed representation of our 2D-input array. This part is further illustrated on the upper-left side of Figure~\ref{fig:model}. For brevity of explanation, we consider a single query vector $[\q]_{i,j}\in{\Q}$ and key vector $[\k]_{i',j'}\in{\K}$, while in practice, this operation is performed for every $i,i' \in [1,\ldots,N]$ and $j,j' \in [1,\ldots,C]$.

First, we compute the following three attention scores (where $T$ here denotes the matrix transpose operation): %\hr{the indexing of m,r is unclear to me. note I changed l-->m since l is used as session index. Actually, why not just use notations i',j'?}\us{I think its a good idea. looks better now? There was a slight mistake, fixed it.}

$$\A_{i, j, i', j'}^{F} = [\q]_{i, j} \cdot [\k]^T_{i', j'},\ \
\A_{i,i'}^{I} = \sum_{z=1}^C [\q]_{i, z} \cdot [\k]^T_{i', z},$$
$$\A_{j,j'}^{C} = \sum_{z=1}^N [\q]_{z, j} \cdot [\k]^T_{z, j'},$$ 

where:
%\begin{enumerate}

\noident $\bullet$ \textbf{$\A^F$} is a 4D-array of attention scores between all inputs as the dot-product between every query vector and every key vector. This attention corresponds to the attention scores in a vanilla attention layer between any two tokens, yet with the distinction that in our case we have 2D-inputs.

\noident $\bullet$ \textbf{$\A^I$} 
 is a matrix of attention scores between whole items in our input, computed as the marginal attention over all channels. This attention captures the importance of items to each other regardless of a particular channel. %, similar to the motivation in the vanilla attention assuming only item representations are considered. %\ye{didn't get the last clause} \hr{Uriel, check my update.."assuming...", I think this should clarify Yotam's comment}

\noident $\bullet$ \textbf{$\A^C$} 
is a matrix of attention scores between channels in our input, computed as the marginal attention over all items. This attention captures the importance of channels to each other regardless of a particular item.

%\end{enumerate}

The attention scores are further combined using their weighted sum: $\A_{i, j, i', j'} = \alpha_1 * \A^F_{i, j, i', j'} +  \alpha_2 * \A^I_{i,i'} + \alpha_3 * \A_{j,j'}^{C},$
where $\alpha_1,\alpha_2,\alpha_3$ are learned scalars, denoting the relative importance of each attention variant, respectively.

The result of this step is, therefore, a 4D-array $\A$ of attention scores from any position $(i,j)$ to every position $(i',j')$. Similarly to \cite{vaswani2017attention},
we apply a softmax function over $\A$,\footnote{For that, we flatten the last two dimensions and treat it as one long vector.} with a scaling factor of $\sqrt{d}$, so that our scores will sum up to 1.  We then compute the final transformed output $[\o]_{i,j}$ as a weighted average over all value vectors using the computed attention scores:

$$\P = softmax\left(\frac{A}{\sqrt{d}}\right) \quad ; \quad [\o]_{i, j} = \sum_{i', j'} \P_{i, j, i', j'}[v]_{i', j'} $$

Finally, we can define our \Atd layer as an attention layer that a receives a triplet of $(\Q, \K, \V)$ 2D-arrays of query, key and value vectors as its input and outputs a 2D-array transformed vectors:

\begin{equation}
\begin{split}
\AtdH(\Q, \K, \V) = [\o]_{i, j} \\ i \in [1,\ldots,N], j \in [1,\ldots,C]
\end{split}
\end{equation}

The \Atd layer allows each item-attribute to attend to all possible item-attributes in the input. To prevent unwanted attendance (such as accessing future information in the sequence), we mask it out by forcing the relevant (future) attention values to $-\infty$ before the softmax operation.

\subsubsection{Multi-Head \Atd}
\label{sec:multihead}
Similarly to~\cite{vaswani2017attention}, instead of performing a single attention function, we can apply $h$ different functions (``Attention-Heads'') over different sub-spaces of the queries, keys, and values. This allows to diversify the attention patterns that can be learned, helping to boost performance. For instance, one attention head can learn to focus on price-seller patterns, while another can find a different price-condition pattern.
We facilitate this by applying $h$ different \Ltd layers, resulting in $h$ triplets of  $(\Q_r, \K_r, \V_r)$.
On each triplet we apply the aforementioned \AtdH layer. % \ref{sec:tensordot}. 
We then concatenate all $h$ results and project it back to a $d$-dimensional vector using another \Ltd layer, as follows:
\begin{equation}
\begin{split}
\MHtd(\Q, \K, \V) = \Ltd_{W^O}(Concat(head_1,...,head_h)) \\
head_r = \AtdH(\Q_r, \K_r, \V_r) \\
\Q_r = \Ltd_{Q_r}(\Q) \ ; \ \K_r = \Ltd_{K_r}(\K) \ ; \ \V_r = \Ltd_{V_r}(\V) \\
\end{split}
\end{equation}

\subsubsection{Position-wise Feed-Forward Networks}
We finally allow the \Atd output to go through additional \Ltd layers in order to be able to cancel out unwanted applied alignments and learn additional complex representations: % \hr{Uriel, note I change to ReLU}:

% $$FFN(\X) = \Ltdb_{W^2,b^2}(max(0, \Ltdb_{W^1,b^1}(\X)))$$

$$FFN(\X) = \Ltdb_{W^2,b^2}(ReLU( \Ltdb_{W^1,b^1}(\X)))$$

\subsubsection{Full Layer implementation}
A full \Atd block is combined from a \MHtd layer and then a FFN layer, where a residual connection \cite{he2016deep} is applied around both, by adding the input to the output and applying a layer normalization \cite{ba2016layer}, as follows:

\begin{equation}
\begin{split}
\Atd(\X)=LayerNorm(\X'+FFN(\X')), \\ \X'=LayerNorm(\X+\MHtd(\X, \X, \X))
\end{split}
\end{equation}


After applying the \Atd block, we end up with a transformed 2D-array of vectors $\X'=\Atd(\X)$, having the same shape as the original input. Therefore, \Atd layers can be stacked one on the other to achieve deep attention networks.

\subsection{Output Layer}
The final stage in our model is label prediction. At this stage, we hold a 2D-array of vectors $\E' = [\e']_{i, j}$ -- a transformed representation of $\E$, the output of the embedding layer (see again Section~\ref{sec:embedding}).
In order to have a single representation for each item, we apply a pooling layer over the channel dimension. While many pooling options may be considered, we used a simple average pooling. 
This is similar to the channel dimension reduction discussed in Section~\ref{sec:modified_transformer}, but %\ye{*crucially*,} \hr{Yotam, please clarify your comment here?} \ye{wanted to suggest adding the word 'crucially' as this is the main idea of attention2D} 
instead of applying the pooling before the attention mechanism, we are able to apply the pooling after the \Atd block. This makes it possible for the \Atd block to capture better attention patterns between different items and attributes.
We then apply a simple fully connected layer to a single neuron representing the probability of an item being clicked:

\begin{equation}
\begin{split}
\hat{y}=\sigma(\W_p \cdot Pool(\E') + b_p) 
\end{split}
\end{equation}

Where $\W_p \in \RR^{d \times 1}; b_p \in \RR$ are trainable parameters, $\sigma(\cdot)$ is the sigmoid activation, and $Pool(\cdot)$ is any pooling operation over the channel dimension, chosen in our case to be average-pooling.

During \textbf{training}, each \wl snapshot $\WL_{t+1}$ is given as a sample together with its historical sequence $\H(t)$ ($0\leq{t}\leq{T_u}-1$) and binary cross-entropy loss is applied only over the given \wl snapshot. %\ye{this might need a rephrase. Not clear what is 'only over the given \wl snapshot' + Not sure Binary CE is *applied* is a correct term... it is the loss function that is minimized} \hr{I understand Yotam's confusion here....we should define this part in terms of $S(t)$ and $\WL_{t+1}$} 
The final loss is, therefore: 
\begin{equation}
    Loss = \sum_{u \in \U}\sum_{t=0}^{T_u-1}\sum^{m^u_{t+1}}_{i=1} Loss^u_{t+1,i}
\end{equation} 
where: $Loss^u_{t+1,i} = - \left[ {y^u_{t+1,i} log(\hat{y}^u_{t+1,i}) + (1-y^u_{t+1,i}) log(1-\hat{y}^u_{t+1,i})} \right] $.

%\ye{consider: it might be simpler(not sure?) to refer to each item in each watch session as a sample. Then move the 3rd summation from $Loss^u_t$ to Loss. Then it is clear this is just regular binary cross entropy} \ye{this last comment of mine is probably incorrect because of the weighting term in $Loss^u_t$. If so, delete it :)}

At \textbf{inference}, we simply concatenate the new RVI items ($\VI_{T_u}$) and \wl snapshot items ($\WL_{T_u+1}$), resolving us with $S(T_u+1)$. We then recommend the top-$k$ items that received the highest predicted click likelihood in $\hat{y}_{T_u+1}$.



==> results.tex <==
\subsection{Main Results}
\begin{table}[]
\caption{\label{table:main}Main results. Boldfaced results indicate a statistically significant difference.}
\center\setlength\tabcolsep{3.0pt}
\small
\begin{tabular}{|l|ccc|cc|cc|} 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \multicolumn{3}{c|}{Precision@k}                 & \multicolumn{2}{c|}{HIT@k}      & \multicolumn{2}{c|}{NDCG@k}      \\ 
\cline{2-8}
\multicolumn{1}{|c|}{}                       & @1             & @2             & @5             & @2             & @5             & @2             & @5              \\ 
\hline
\textbf{\textbf{\Ttd}}  (our model)     &        \textbf{43.51} &        \textbf{33.30} &        \textbf{21.56} &  \textbf{62.19} &  \textbf{80.85} &   \textbf{35.61} &   \textbf{26.12} \\
$\gru_C$    &        39.08 &        31.52 &        21.24 &  58.76 &  79.43 &   33.23 &   25.07 \\
\bst        &        38.15 &        31.21 &        21.28 &  58.09 &  79.57 &   32.78 &   24.94 \\
$\fdsa^-$   &        37.84 &        31.03 &        21.14 &  57.80 &  78.91 &   32.57 &   24.76 \\
$\fdsa^+$   &        36.95 &        30.37 &        21.01 &  56.57 &  78.35 &   31.86 &   24.46 \\
$\trans_T$  &        36.77 &        30.83 &        21.18 &  57.37 &  79.12 &   32.17 &   24.62 \\
\ca         &        36.06 &        30.50 &        21.09 &  56.78 &  78.70 &   31.76 &   24.41 \\
$\trans_A$  &        36.01 &        30.42 &        21.10 &  56.56 &  78.72 &   31.68 &   24.41 \\
$\gru_A$    &        35.71 &        30.41 &        21.08 &  56.58 &  78.65 &   31.61 &   24.35 \\
\lc         &        35.64 &        30.29 &        21.08 &  56.36 &  78.65 &   31.50 &   24.32 \\
\cdmf       &        32.71 &        28.15 &        20.41 &  52.10 &  75.30 &   29.18 &   23.15 \\
\seqfm      &        32.22 &        27.81 &        20.32 &  51.45 &  74.90 &   28.81 &   22.97 \\
\RSP        &        31.44 &        27.82 &        20.17 &  51.43 &  74.16 &   28.64 &   22.73 \\
\price (high to low)      &        15.51 &        15.69 &        15.57 &  27.96 &  52.60 &   15.65 &   15.60 \\
\price (low to high)      & 14.11          & 14.38          & 14.62          & 25.35          & 47.99          & 14.32          & 14.51 \\

\hline
\end{tabular}
\end{table}

We report the main results of our evaluation in Table~\ref{table:main}, where we compare our \textbf{\Ttd} model to all baselines. As can be observed, \textbf{\Ttd} outperforms all baselines over all metrics by a large margin. We next notice that, the best baselines after \textbf{\Ttd} are $\gru_C$ and \bst (Transformer-based). Common to both baselines is the fact that they apply a concatenation over the attribute embeddings. While there is no dimensional reduction in the attribute representation, there are still two drawbacks in such baselines. First, the semantic difference between the attributes is not kept; and therefore, the attention cannot be per attribute. Second, the number of parameters in these baselines drastically increases. \textbf{\Ttd}, on the other hand, %This compared to \textbf{\Ttd} that 
requires only a slight expense of parameters.

Among the next best baselines, are those that employ a Transformer/Attention pooling (i.e., $\trans_T$, $\fdsa^-$, and $\fdsa^+$). Next to these are those that use average-pooling (i.e., $\trans_A$ and $\gru_A$). These empirical results demonstrate that, the attribute reduction mechanism is important to avoid losing important attribute information before entering the sequence block. Therefore, \textbf{\Ttd}, which does not require any such reduction in the attribute representations, results in overall best performance. 

Observing the difference between $\fdsa^+$ (as the only baseline that uses the original item-IDs) and $\fdsa^-$, further shows that using the original \emph{item-ID} resolves in worse results, as it causes an over-fit. This helps verifying the importance of representing items based on their (less sparse) attributes. Furthermore, it is worth noting that, using the \textbf{original} \emph{item-ID} as an attribute harms the performance of all other baselines as well.  Therefore, we implement all other baselines in this work (including our own model) without the original \emph{item-ID} attribute (yet, still with its hashed version).

\begin{figure*}
    \centering
    \subfloat[\# Blocks ($L$)]
        {\includegraphics[width=0.2\textwidth]{Blocks.pdf}}
    \subfloat[\# Heads ($h$)]
    	{\includegraphics[width=0.2\textwidth]{Heads.pdf}}
    \subfloat[Embedding Size ($d$)]
    	{\includegraphics[width=0.2\textwidth]{EmbeddingSize.pdf}}
    \subfloat[Sequence Length ($N$)]
        {\includegraphics[width=0.2\textwidth]{SequenceLength.pdf}}
    \subfloat[Days Considered]
    	{\includegraphics[width=0.2\textwidth]{DaysConsidered.pdf}}
    % \quad
    % \vskip\baselineskip
    \caption{\label{fig:sensitivity}Parameter Sensitivity results. Y-axis represents $NDCG@5$, while similar trends are observed for all other metrics.} %Sequence Length or Days Considered of $0$ represent only considering the last \wl snapshot.}
\end{figure*}

We next observe that, the context-aware baselines (i.e., \ca and \lc) perform similar to the average-pooling baselines. Here we note that, these baselines also perform average-pooling over the context-features (also referred to as the ``next item features''). 
This supports our choice of adding the next possible item to the end of the sequence. Such a choice results in a similar effect to the context-aware approach that adds the item's features as context not before the sequence (GRU) block is applied. Moreover, since we have a relatively small recall-set in our setting, it is possible to concatenate the predicted item features to the history sequence and leverage the \textbf{\Atd} block to encode also the recall-set item attributes together with the sequence. %\hr{Uriel, not really clear...and sounds like a speculation} Assume, in a different setup, we have a large recall-set, the context-aware approach can still be used with \textbf{\Atd} as the base sequence block.

Finally, we can observe that, ordering by the \RSP attribute results in a reasonable baseline on its own. This in comparison to both \price baselines that only provide a weak signal. This implies that, over our sampled users, the price does not pay a big deal, but rather the short-term interactions. This fact is further supported in our next parameter sensitivity analysis, see Figure~\ref{fig:sensitivity}(e). %in\us{add cross-ref support for the sensitivity result of `days considered`?} 

\subsection{Parameter Sensitivity}
\label{sec:parameter_sensitivity}


%\hr{TODO: we need to update based on results with other baselines. To save space, given that most other baselines will behave bellow our curves (with BST exceptional for blocks but we have a citation to confirm this), we can just state that the trend is similar in most cases.}

To better understand how the \textbf{\Ttd} model parameters influence its performance, we check its sensitivity to five essential parameters: 1) $L$, number of attention blocks, 2) $h$, number of heads used in the attention mechanism, 3) $d$, each attribute embedding size, 4) $N$, maximum sequence length, and 5) maximum number of days (back) to be considered in the sequence.
For each parameter sensitivity check, we set the rest to their default values (i.e., $L=1$, $h=4$, $d=16$, $N=50$, and days=`Full History' -- all days are being considered). %, meaning no cutoff has been applied).

We report the sensitivity analysis results (using NDCG@5) in Figure~\ref{fig:sensitivity}. For reference, we also report the sensitivity of the three next best baselines: $\gru_C$, $\bst$ and $\fdsa^{-}$. In general, we can observe that, in the majority of cases, our model outperforms the baselines. Furthermore, almost in all cases, the other baselines  behave similarly to our model. Per parameter, we further make the following specific observations about our model's sensitivity: 
%\us{I removed the `noident` commands as they create errors and I don't see any difference}

\textbf{\# Blocks} ($L$): We notice that, adding a second \textbf{\Atd} block on top of the first helps to learn second-order dependencies. This makes sense, as the two attention matrices of the model, $\A^I$ and $\A^C$, can capture attention only in the same row or column. The only attention type that can capture dependencies between two cells not in the same row or column is $\A^F$. Yet, during the attention calculation on $\A^F$, the cells are not aware of the other values in their row or column. Therefore, a second block is able to capture such second-order dependencies %(i.e., $(i_1,j_1) \rightarrow (i_1,j_2) \rightarrow (i_2,j_2)$) \us{maybe we should give an example, such as price of a given seller can influence the price of another seller..} \hr{indeed}. 
(e.g., price comparison of two different appearances of the same item or leaf-category). %two items from the same leaf-category but have a different price \hr{Uriel, what do you think?} \us{great! if we really want to give intuition, we can give an additional example: different price of the same item-ID, different item-condition from the same seller-ID, price of same item from different site-ID's, etc..}). 
We can further observe that, the third block has less influence on performance. %\us{add cross-ref for the ablation $-\A^F$. the ablation is not that important, but it might when $L=2$..?}
Finally, %among the baselines, 
similar to the results reported in~\cite{10.1145/3326937.3341261}, with additional blocks, $\bst$'s performance actually declines. %behaves differently, where additional attention blocks decline its performance. %\footnote{A similar behavior was previously reported by $\bst$ authors~\cite{10.1145/3326937.3341261} (see Table 4).}.

\textbf{\# Heads} ($h$): Similar to normal attentions, utilizing more heads enables the attention mechanisms to learn multiple patterns. 
Here, we explore two main options for head sizes: 1) each head size equals the input size or 2) all head sizes together equal the input size. For our model and $\fdsa^{-}$ the first option is better, while for $\bst$, the second option is better. For the latter, this can be explained by its already over-sized input and data sparsity (see further details next in Embedding Size sensitivity). 
Overall, we observe that, $4$ heads resolves with a good performance, while $5$ heads already has a minor impact on our model's performance. %\hr{I removed this} We note that, these results are relevant specifically to our dataset, while more/less heads might help boost results over other datasets.
%\us{While in our paper, for all baselines, each head size equals to the input size, it can harm the performance of \bst, as the input size is large and sparse (as demonstrated and discussed next paragraph). Therefore, for \bst, we experimented with the following two approaches: 1) each head size equals to the input size (similar to our model and all other baselines), and 2) all head sizes together are equal to the inputs size. As expected, due to sparsity, the latter performed better. Therefore, all \bst results reported in this paper are with the second approach.}

\textbf{Embedding Size} ($d$): 
%We first observe that, 
Interestingly, for our model, an embedding size of $d=32$ resolves with the best performance. While the trend for $d<32$ can be explained by too small representation sizes, the interesting trend is for $d>32$. This can be explained due the vocabulary size of each attribute. While most attributes include only few or tens of unique values, only \emph{user-ID}, \emph{level1-category}, and \emph{leaf-category} hold $40,344$, $1,293$, and $25,449$ unique values, respectively. Therefore, while a larger representation may help the latter, the rest of the attributes suffer from over-representation and sparsity. We note that, those baselines that use concatenation ($\gru_C$ and \bst) can be thought as using a larger representation for each item. This fact supports the performance decline we observe for these baselines: with larger representations, more over-fit. Differently from the former two, $\fdsa^{-}$ actually manages to improve (up to some point)  with the increase in embedding size. We attribute this to its usage of the vanilla attention pooling over the attribute embeddings, which in turn, allows it to represent attributes together in an efficient way, even if some are very sparse. 


%\hr{I remove this to save space} Finally, we believe that, being able to handle different attribute embedding sizes may help improve performance. We leave such a direction for future work. 

\textbf{Sequence Length} ($N$) + \textbf{Days Considered}:  The result of the \RSP baseline implies that, users' \wl priorities are usually driven by short-term patterns. Such patterns are captured by users' recently viewed item pages. We can observe that, 
for both parameters, $N=50$ or $days=1$ is enough in order to capture most of the important short-term signal. We further see a small improvement in extending the time range or sequence length. This implies that there is still a weak signal that can be captured. %We note that, 
Since the sequence model is a Transformer, there is no memory-gate involved (like in GRU); hence, these short-term patterns represent a real user-behaviour.


\subsection{Ablation Study}


We next perform an ablation study and report the results in Table~\ref{table:ablation}. To this end, every time, we remove a single component from the \textbf{\Ttd} model and measure the impact on its performance. We explore a diverse set of ablations, as follows: 
%For the ablation studies reported in Table \ref{table:ablation}, we removed the following components separately from the full implementation of the \textbf{\Atd} model:

$-\Ltd$: We switch every \Ltd layer with a \Lod layer, meaning all channels receive the exact same weights. This ablation allows to  better understand the importance of the attribute-alignment.
While this modified component downgrades performance, it still outperforms all baselines while keeping the exact same number of parameters as in a regular attention layer (except for the three $\alpha$ scalars used in Eq.~\ref{eq:final_attn}). This confirms that, the improvement of the full \textbf{\Ttd} results are not only driven by the \Ltd layer but also by the attention mechanism itself.

$-\A^F$,$-\A^C$,$-\A^I$: We remove each one of the three attention parts from the final attention calculation in Eq.~\ref{eq:final_attn}. These ablations allow to better understand the importance of each attention type to the full model implementation.
%From the results, we derive that, the 
The most important attention part is $\A^I$, %This makes sense, as this attention type is the attention between any two items as done in a regular attention layer. 
showing that the relationship between user's items is the most important, following the motivation of the 1D-attention mechanism.
$\A^I$ is followed by $\A^C$ and then by $\A^F$. As we can further observe,  $\A^F$ does not hold significant importance. We hypothesis that, while $\A^F$ is the only attention part that can capture dependencies between two cells not in the same row or column, during the attention calculation on $\A^F$, the cells are not aware of the other values in their row or column. This can be over-passed by adding an additional \textbf{\Atd} layer, as shown and discussed in Section~\ref{sec:parameter_sensitivity} over the \# Blocks sensitivity check, see again Figure~\ref{fig:sensitivity}(a).

$-RVI,-\wl$: We remove from the history sequence all items having \emph{interaction type}=RVI (item-page-view) and \emph{interaction type}=\wl (click), respectively. These ablations allow to understand the importance of each \emph{interaction type} to the WLR task.
%We observe that, 
While both are important, \wl clicks hold a stronger signal. This actually makes sense: while item page views (RVIs) provide only implicit feedback about user's potential interests, %(\wl)
clicks provide explicit feedback that reflect actual user \wl priorities. 

\begin{table}[]
\caption{\label{table:ablation}Ablation results. Starting from the second row, on each, a single component is removed from the model. }%\us{we need to see want to do with the problematic ablations}}
\center\setlength\tabcolsep{3.0pt}
\small
\begin{tabular}{|l|ccc|cc|cc|} 
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model ~}}        & \multicolumn{3}{c|}{Precision@k}                 & \multicolumn{2}{c|}{HIT@k}      & \multicolumn{2}{c|}{NDCG@k}      \\ 
\cline{2-8}
\multicolumn{1}{|c|}{}                                & @1             & @2             & @5             & @2             & @5             & @2             & @5              \\ 
\hline
\textbf{\textbf{\Ttd}}  (our model)     &        43.51 &        33.30 &        21.56 &  62.19 &  80.85 &   35.61 &   26.12 \\
% -negatives         & 42.71          & 32.79          & 21.42          & 61.19          & 80.22          & 35.03          & 25.85           \\
-$A^F$            &        44.01 &        33.42 &        21.56 &  62.42 &  80.85 &   35.82 &   26.20 \\
% -current           & 42.52          & 32.73          & 21.44          & 61.09          & \textbf{80.29} & 34.95          & 25.83           \\
-time             &        43.25 &        33.17 &        21.55 &  61.93 &  80.79 &   35.45 &   26.06 \\
-RVI              &        43.21 &        33.09 &        21.51 &  61.81 &  80.62 &   35.38 &   26.01 \\
-$A^C$            &        43.03 &        33.06 &        21.53 &  61.72 &  80.69 &   35.32 &   26.00 \\
-item             &        42.21 &        32.64 &        21.40 &  60.89 &  80.13 &   34.80 &   25.74 \\
-Linear2D         &        41.93 &        32.71 &        21.50 &  61.02 &  80.56 &   34.80 &   25.79 \\
-\wl              &        40.07 &        31.48 &        21.08 &  58.56 &  78.49 &   33.42 &   25.08 \\
-$A^I$            &        38.83 &        31.60 &        21.36 &  58.84 &  79.92 &   33.24 &   25.14 \\
-history          &        33.04 &        28.45 &        20.46 &  52.66 &  75.53 &   29.49 &   23.27 \\
-position         &        32.18 &        26.77 &        19.86 &  49.45 &  72.81 &   27.99 &   22.51 \\
\hline
\end{tabular}
\end{table}

%This demonstrates the importance of analysing the journey of a user with his \wl. \hr{how come? -watchlist cause higher drop in performance!} \us{you're right, my bad. better now?} \hr{no, now its sounds like hand-waving...there are two observations here. First, click is explicit interest vs. view which is implicit so it will always carry more signal of user's preference. Second, RVIs drop proves the fact that we claimed that user's interest is also driven by such events. I will modify to reflect this...}
% This can be explained by the fact that the user first views related items' pages, which in its turn, makes her click an item in her \wl (e.g., the clicked item has an attractive price). This in contrast to previous \wl items that the user may have already lost interest in \hr{speculation...not sure this is true...actually, a very strong signal should have been repetitive item clicks!...I suggest to remove this last sentence} (e.g., as they got already clicked or purchased).

$-time,-item,-position$: For each, we remove a group of attributes in order to better understand the importance of the attributes to the WLR task. For $-time$, we remove the \emph{hour}, \emph{day}, and \emph{weekday} attributes. For $-item$, we remove the \emph{price}, \emph{condition}, \emph{level1-category}, \emph{leaf-category}, and \emph{sale-type} attributes. For $-position$, we remove the \emph{position-ID}, \emph{relative-snapshot-position} (\RSP), \emph{snapshot-ID}, \emph{hash-item-ID}, and \emph{hash-seller-ID} attributes.
Examining the ablations results, shows that the most important attribute-set is the position-set, followed by the item-set, and finally by the time-set. Noticing that the position-set includes \RSP explains their high importance. The time-set is not that important as relative-time is encoded in the position-set. Additionally, the dataset spans over a relatively short period, resolving with less data to learn the importance of a specific weekday, hour of the day, or day of the month.

$-history$: To understand the importance of the entire history, we remove all the history sequence, and solely predict over $\WL_t$ -- the last snapshot.
We see that, not observing any history, drastically harms the performance of the model. This strengthens the argument that considering user's history is important for the WLR task. %sequence-based recommendation is an important setup for recommendation tasks, and specifically for the WLR task.

\subsection{Qualitative Example}

\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{Qualitative2.pdf}
\caption{Qualitative Example. For brevity, only 6 out of the 16 possible attributes are presented. The darker the item-attribute cell color is, the more important it is. %`Null` has a special token per attribute representing missing values.  
The current candidate is surrounded with the black rectangular. 
}
\label{fig:qualitative}
\end{figure}

We end this section with a qualitative example (see Figure~\ref{fig:qualitative}) that visualizes the attention values assigned by the \textbf{\Ttd} model to items' attributes in a given user-sequence. The last item in the sequence is the \wl item for which the model makes a prediction. This item is actually clicked by the user ($y=1$) and the model's prediction is aligned, assigning it the highest likelihood amongst all \wl snapshot items ($\hat{y}=0.697$).

As the learned attention is a 4D-array, representing the attention between any two (item,attribute) pairs (see Section~\ref{sec:tensordot}), we first pick the attention over the last item in the sequence, and then average over the channel dimension. Doing so, resolves us with a 2D-array that can be visualized to better understand the importance of each (item,attribute) pair on the prediction of the item.  Observing the channel dimension, we can notice that, different attributes have different importance. This strengths the importance of a 2D-attention that is able to learn the attention over a second axis.

As we can observe, given the next item to predict, the model emphasizes either previously clicked items related to the current predicted item (e.g., leaf-categories: 8159--`\texttt{Home Security:Safes}`, 4895--`\texttt{Safety:Life Jackets \& Preservers}`) or RVIs that belong to the same leaf-category of the current item (8159). Interestingly, the model emphasizes the prices of clicked items in the same leaf-category (8159), which are higher than the predicted item's price. 

